Expiring Assets in Automated Market Makers

An automated market maker (AMM) is a state machine that manages pools of assets, allowing parties to buy and sell those assets according to a fixed mathematical formula. AMMs are typically implemented as smart contracts on blockchains, and its prices are kept in line with the overall market price by arbitrage: if the AMM undervalues an asset with respect to the market, an "arbitrageur" can make a risk-free profit by buying just enough of that asset to bring the AMM's price back in line with the market. AMMs, however, are not designed for assets that expire: that is, assets that cannot be produced or resold after a specified date. As assets approach expiration, arbitrage may not be able to reconcile supply and demand, and the liquidity providers that funded the AMM may have excessive exposure to risk due to rapid price variations. This paper formally describes the design of a decentralized exchange (DEX) for assets that expire, combining aspects of AMMs and limit-order books. We ensure liveness and market clearance, providing mechanisms for liquidity providers to control their exposure to risk and adjust prices dynamically in response to situations where arbitrage may fail.

==> old_versions/loss_control.tex <==
With the above price adjustment protocol, liquidity providers can face a significant loss, called \emph{divergence loss}. Each liquidity provider will tolerate some amount of risk, which we measure as divergence loss. In particular, if some liquidity provider's divergence loss ever exceeds a certain value, a rational liquidity provider will temporarily remove their liquidity until the computed divergence loss falls within the tolerated loss. Thus the more risk-averse liquidity providers have a greater potential loss, but they will receive more fees as they are \emph{active} for more of the trades.

Our \emph{divergence loss control} protocol automates this idea for liquidity providers, which reduces unnecessary gas fees and does not require liquidity providers to constantly observe the AMM state. First, let us formally define divergence loss.


Let $\ell \in L$. Suppose $(x_0, y_0)$ was the liquidity state immediately after $\ell$ joined the set $L$, and suppose $c_0$ was the aggregate constant at that time, call it $t_0$. Suppose the current state is $(x,y)$ and the current constant is $c$, at time $t > t_0$ with $t \in T$. Let $s_{\ell, 0}$ be the share of $\ell$ at time $t_0$ and let $s_\ell$ be the current share of $\ell$, at time $t$. Let $p_0 = |f'_{c_0, (x_0,y_0)}(x_0)|$ and $p = |f'_{c, (x, y)}(x)|$ be the instantaneous prices per unit of $Y$ at times $t_0$ and $t$, respectively. Define the \emph{divergence loss} at time $t$ to be
\begin{align*}
DL(\ell) &= s_{\ell, 0} \cdot (x_0 + p_0\cdot y_0) - s_\ell \cdot (x + p\cdot y)\\
&= s_{\ell, 0} \cdot (x_0 + c_0 y_0/x_0)  - s_\ell \cdot (x + cy/x).
\end{align*}
The liquidity provider $\ell$ accrues a loss if $DL_{\ell} > 0$. Of course, with this definition, divergence loss can decrease simply when the liquidity providers collectively increase the aggregate constant $c$ over time. Thus, a liquidity provider is defined as a user that is willing to tolerate divergence loss in exchange for fees.

In a standard AMM with a fixed curve and nonperishable assets, divergence loss is typically defined in terms of the market \emph{valuation} of the two assets, where the market valuation describes the respective value of the assets in terms of the other. However, our curve is not fixed and there is typically not a single valuation of the assets that all participants share. Differently, buyers can value the perishable asset arbitrarily. As a consequence, we cannot use valuations to define divergence loss to liquidity providers, so we use the current state of the AMM (in particular, the price) to approximate the average market valuation over all costumers.


Now we finally describe our divergence loss control protocol.
When the AMM is initialzed, it initializes two sets, $L$ and $L'$, where $L$ represents the set of \emph{active} liquidity providers, and $L'$ represents the set of \emph{inactive} liquidity providers. The set $L$ initially only contains the owner of the AMM and the set $L'$ initially is empty. We also keep track of maps $m_X: L \cup L' \to \R_{\ge 0}$ and $m_Y: L' \to \R_{\ge 0}$ initialized as empty maps. Any undefined value is set to $0$, such as when a liquidity provider first joins the set $L$.

Each liquidity provider initially publishes a value $d_\ell \ge 0$, which represents an approximate upper bound on divergence loss. At each time $t \in T$, we do the following. Update the state curve as per usual. Remove all $\ell \in L$ such that $DL(\ell) > d_\ell$ from $L$ and add them to $L'$. For each such $\ell$, set $m_X(\ell) = s_\ell x$ and $m_Y(\ell) = s_\ell y$. Readjust the values of $s_\ell$ for $\ell \in L$ and update the current state $(x,y)$. Update the aggregated $c$ and then the state curve again. For each $\ell \in L'$ that was added to $L'$ at a time before $t$, if $c_\ell \ge c$, then we add $\ell$ to $L$ and do the following; if $m_X(\ell) / m_Y(\ell) \ge x / y$, then do $y \gets y + m_Y(\ell)$, $x \gets x + (xm_Y(\ell)/y)$, $m_Y(\ell) \gets 0$, $m_X(\ell) \gets m_X(\ell) - (xm_Y(\ell)/y)$; otherwise, $m_X(\ell) / m_Y(\ell) < x / y$, then do $x \gets x + m_X(\ell)$, $y \gets y + (ym_X(\ell)/x)$, $m_X(\ell) \gets 0$, $m_Y(\ell) \gets m_Y(\ell) - (ym_X(\ell)/x)$; if after doing these computations we have $DL(\ell) > d_\ell$, revert these changes and continue to the next member of $L'$. Remove the now active liquidity providers from $L'$ by doing $L' \gets L' \setminus L$. Finally, update liquidity shares $s_\ell$ for all $\ell \in L \cup L'$ (set $s_\ell = 0$ if $\ell \in L'$), the aggregate $c$, and the state curve.\\




How much does divergence loss change as a given liquidity provider $\ell$ changes $c_\ell$? This is measured precisely by the partial derivative of $DL_\ell$ with respect to $c_\ell$:
\begin{align*}
    \frac{\partial (DL_\ell)}{\partial c_\ell} &=
    s_\ell \cdot \frac{\partial}{\partial c_\ell} (x + y|f'_{c, (x,y)}(x)|)\\
    &= s_\ell \cdot \frac{\partial}{\partial c_\ell} \left(x - y \left.\frac{d}{dx'}\left(y (x'/x)^{-\prod_{\ell' \in L} c_{\ell'}^{s_{\ell'}}}\right)\right|_{x' = x}\right)\\
    &= s_\ell \cdot \frac{\partial}{\partial c_\ell} \left(x - y \left.\left( -\frac{y}{x} \prod_{\ell' \in L} c_{\ell'}^{s_{\ell'}} \cdot (x'/x)^{-\prod_{\ell' \in L} c_{\ell'}^{s_{\ell'}}-1} \right)\right|_{x'=x}\right)\\
    &= s_\ell \cdot \frac{\partial}{\partial c_\ell} \left(x - y \left( -\frac{y}{x} \prod_{\ell' \in L} c_{\ell'}^{s_{\ell'}} \right)\right)\\
    &= s_\ell \cdot \left( \frac{y^2}{x} \cdot s_\ell c_\ell^{s_\ell - 1} \cdot \prod_{\ell' \in L\setminus\{\ell\}} c_{\ell'}^{s_{\ell'}} \right)\\
    &= s_\ell \cdot \left( \frac{y^2}{x} \cdot s_\ell/c_\ell \cdot \prod_{\ell' \in L} c_{\ell'}^{s_{\ell'}} \right)\\
    &= \frac{y^2 s_\ell^2 c}{x c_\ell}.
\end{align*}
This computation shows exactly how much control a given liquidity provider has over their own divergence loss.


What about other measures of loss to liquidity providers? Liquidity providers face more than simply divergence loss; they face the perishability of one of the assets. At expiration, the value of all units of the perishable asset drop to $0$.\\


Here is an alternative formulation of loss that incorporates the order book, rather than instantaneous prices. The advantages of this approach are that it sheds light on the current demand for the perishable asset, and mitigates the possibly chaotic changes in instantaneous price due to changes in the aggregate constant $c$. We assume that all bids (orders) are locked. That is, if a user places an order for a price $p$, that user cannot withdraw the order, nor decrease its price to any $p' < p$, however, the user can increase the price of the order to any $p' > p$ at any time. Let $\ell$ be any liquidity provider. Let $(x_0, y_0)$ be the liquidity state at the time $\ell$ joined the pool, where $\ell$ has a share of $s_{\ell,0}$; let $\mathcal{O}_0$ be the set of orders at this time, where an order is a pair $(u, p)$ such that $u$ is the user that submitted the order for a price $p$. Let $(x,y)$ be the current liquidity state, where $\ell$ has a share $s_{\ell}$; let $\mathcal{O}$ be the current order set. Since liquidity providers are dynamic participants, we may not assume $s_\ell = s_{\ell, 0}$. Given an order book $\mathcal{O}$ and some $o = (u,p) \in \mathcal{O}$, let $\mathtt{secondPrice}(o; \mathcal{O})$ to be maximum $p' \le p$ such that some order in $\mathcal{O} \setminus \{o\}$ has price $p'$; if no such order exists, set $\mathtt{secondPrice}(o; \mathcal{O}) = p$.
Define
\[
\mathtt{minProfit}(x, y; \mathcal{O}) = x + \max\left\{\sum_{o \in \mathcal{O}'} \mathtt{secondPrice(o; \mathcal{O})}: \mathcal{O}' \subseteq \mathcal{O} \wedge |\mathcal{O}'| \le y\right\}.
\]
Finally, we define the \emph{order loss} to liquidity provider $\ell$ at the current time to be
\[
\mathtt{orderLoss}(\ell) = s_{\ell,0} \cdot \mathtt{minProfit}(x_0, y_0; \mathcal{O}_0) - s_\ell \cdot \mathtt{minProfit}(x, y; \mathcal{O}).
\]
According to this metric, liquidity provider $\ell$ is expecting a profit if its order loss is negative.

\todo{Make a function that LPs can call to become inactive or reactivate at any time. Every LP can choose to use this DL control or not, and instead, use the manual inactivation.}
